Adaptable Embeddings Network (AEN)

Modern day Language Models see extensive use in text classification, yet this comes at significant computational cost. Compute-effective classification models are needed for low-resource environments, most notably on edge devices. We introduce Adaptable Embeddings Networks (AEN), a novel dual-encoder architecture using Kernel Density Estimation (KDE). This architecture allows for runtime adaptation of classification criteria without retraining and is non-autoregressive. Through thorough synthetic data experimentation, we demonstrate our model outputs comparable and in certain cases superior results to that of autoregressive models an order of magnitude larger than AEN's size. The architecture's ability to preprocess and cache condition embeddings makes it ideal for edge computing applications and real-time monitoring systems.

==> table/initial_findings/concat_table.tex <==
\newcommand*\concatTable{%
\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Concatenation Method} & \textbf{Train F1} & \textbf{Test F1} \\
\hline
 \( (u, v) \) & 0.925 & 0.914 \\
 \( (|u-v|) \) & 0.850 & 0.920 \\
 \( (u, v, u \cdot v) \) & 0.925 & 0.944 \\
 \( (u, v, |u-v|) \) & 0.920 & 0.937 \\
\( (u, v, |u-v|, u \cdot v) \) & 0.934 & 0.924 \\
\hline
\end{tabular}
\caption{Comparison of different concatenation methods and their performance metrics}
\label{tab:concat_methods_comparison}
\end{table}
}

==> table/initial_findings/encoder_type.tex <==
\newcommand*\encoderTable{%
\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Encoder} & \textbf{Size} & \textbf{Train F1} & \textbf{Test F1} \\
\hline
all-MiniLM-L6-v2 & 384 & 0.920 & 0.937 \\
all-mpnet-base-v2 & 768 & 0.949 & 0.967 \\
\hline
\end{tabular}
\caption{Comparison of different encoder types and their performance metrics}
\label{tab:encoder_type_comparison}
\end{table}}

==> table/initial_findings/ffnn_structure.tex <==
\newcommand*\structureTable{%
\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{FFNN Parameters} & \textbf{Train F1} & \textbf{Test F1}  \\
\hline
299,841 & 0.895 & 0.906 \\
499,393 & 0.922 & 0.913  \\
723,457 & 0.927 & 0.951  \\
2,054,017 & 0.920 & 0.937  \\
3,384,577 & 0.920 & 0.931  \\
\hline
\end{tabular}
\caption{Comparison of different FFNN structures and their performance metrics}
\label{tab:ffnn_structure_comparison}
\end{table}
}

==> table/initial_findings/fine_tune_table.tex <==
\newcommand*\tuneTable{%
\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Type} & \textbf{Train F1} & \textbf{Test F1} \\
\hline
No Fine Tuning & 0.920 & 0.937 \\
Same Encoder Tune & 0.981 & 0.997 \\
Diff Encoder Tune & 0.964 & 0.993 \\
\hline
\end{tabular}
\caption{Comparison of different grad lock configurations and their performance metrics}
\label{tab:grad_lock_comparison}
\end{table}}

==> table/initial_findings/imports.tex <==
% \input{table/concat_table}
% \input{table/ffnn_structure}
% \input{table/encoder_type}
% \input{table/fine_tune_table}
